ClothAtlas: Joint Garment Identification and State Estimation under Self-Occlusion

Garment manipulation requires inferring both garment identity and complete configuration from partial, self-occluded observations. This creates a chicken-and-egg problem: completing a partial observation requires a garment-specific deformation prior, while identifying the garment requires a configuration that explains the observation. We introduce ClothAtlas, which jointly identifies garments and estimates their complete configurations from partial point clouds and a library of canonical meshes. A shared graph-conditioned flow-matching model samples configurations for each candidate mesh and ranks candidates by observation fit. The model accommodates different mesh shapes, vertex counts, and connectivities, allowing new garments to be added from canonical meshes alone without retraining. On held-out DexGarmentLab garments, ClothAtlas ranks the correct mesh first among 221 candidates for all 22 test garments from a single flat observation. From a single self-occluded observation, it identifies 15/22 garments, compared with 8/22 for a deterministic graph estimator. Persistent vertex identities support grasp-target localization on real garments, reducing mean error from 15.4 to 6.4 cm overall and from 17.0 to 8.3 cm on occluded targets compared with dense descriptor matching. Project page: https://clothatlas.github.io/

==> Images/data/reconstruction_violins/chamfer_mm.tex <==
\CPViolin{chamfer_mm_rigid}{0}{cpviolinrigid}{1.44693783634}{2.06071748678}{2.19972719377}{2.30197232307}
\CPViolin{chamfer_mm_completion}{1}{cpviolincompletion}{1.10082149074}{1.20367514617}{1.25478291744}{1.34103964147}
\CPViolin{chamfer_mm_deterministic}{2}{cpviolindeterministic}{1.02270505013}{1.10877430596}{1.15755529597}{1.65560049742}
\CPViolin{chamfer_mm_independent}{3}{cpviolinindependent}{1.0008341687}{1.06923443748}{1.10833660612}{1.22774461072}


==> Images/data/reconstruction_violins/chamfer_occ_mm.tex <==
\CPViolin{chamfer_occ_mm_rigid}{0}{cpviolinrigid}{1.48569772587}{2.0086744936}{2.12032383179}{2.25895434146}
\CPViolin{chamfer_occ_mm_completion}{1}{cpviolincompletion}{1.09173334762}{1.20280493914}{1.26279791499}{1.37595845922}
\CPViolin{chamfer_occ_mm_deterministic}{2}{cpviolindeterministic}{1.02374405096}{1.11414900247}{1.16766777161}{1.65713638033}
\CPViolin{chamfer_occ_mm_independent}{3}{cpviolinindependent}{1.00342347035}{1.0809352788}{1.12454918314}{1.25686913504}


==> Images/data/reconstruction_violins/vert_err_p90_mm.tex <==
\CPViolin{vert_err_p90_mm_rigid}{0}{cpviolinrigid}{2.22236284455}{2.63236512498}{2.73306681622}{2.96011680213}
\CPViolin{vert_err_p90_mm_completion}{1}{cpviolincompletion}{2.066823362}{2.52175274405}{2.66857594789}{2.97044543676}
\CPViolin{vert_err_p90_mm_deterministic}{2}{cpviolindeterministic}{1.24006018881}{1.55705973536}{1.74094449481}{2.70930949533}
\CPViolin{vert_err_p90_mm_independent}{3}{cpviolinindependent}{1.06297150023}{1.40831988736}{1.58187680076}{1.97518891753}


==> Images/fig1/gallery_metadata.tex <==
\def\figonegalleryrows{dress/Dresses/26/1/5/8,tops/Tops/95/1/5/8,trousers/Trousers/100/1/3/6}%


==> Images/fig1/surface_annotation.tex <==
\coordinate (occluded-surface) at (barycentric cs:fitted-nw=-0.307513481,fitted-ne=0.642590700,fitted-sw=0.664922781);


==> Images/fig1/tracking_annotations.tex <==
\coordinate (tracking-camera) at (barycentric cs:tracking-nw=0.569029869,tracking-ne=0.024031774,tracking-sw=0.406938356);
\coordinate (tracking-camera-focus) at (barycentric cs:tracking-nw=0.084883700,tracking-ne=0.120714270,tracking-sw=0.794402030);
\coordinate (tracking-lift-0) at (barycentric cs:tracking-nw=0.107470165,tracking-ne=0.139866790,tracking-sw=0.752663045);
\coordinate (tracking-lift-end-0) at (barycentric cs:tracking-nw=0.269911038,tracking-ne=0.139869268,tracking-sw=0.590219694);
\coordinate (tracking-lift-1) at (barycentric cs:tracking-nw=0.135500750,tracking-ne=0.385195285,tracking-sw=0.479303965);
\coordinate (tracking-lift-end-1) at (barycentric cs:tracking-nw=0.297941622,tracking-ne=0.385197763,tracking-sw=0.316860615);
\coordinate (tracking-lift-2) at (barycentric cs:tracking-nw=0.116137056,tracking-ne=0.633217990,tracking-sw=0.250644954);
\coordinate (tracking-lift-end-2) at (barycentric cs:tracking-nw=0.278577979,tracking-ne=0.633220418,tracking-sw=0.088201604);
\coordinate (tracking-lift-3) at (barycentric cs:tracking-nw=0.061167979,tracking-ne=0.882782753,tracking-sw=0.056049268);
\def\figonetrackingcameraangle{-53.346180}


==> Images/reconstruction_ranks/values.tex <==
\expandafter\def\csname rrScoredeterministic1\endcsname{11.49}%
\expandafter\def\csname rrScoredeterministic2\endcsname{12.14}%
\expandafter\def\csname rrScoredeterministic3\endcsname{12.48}%
\expandafter\def\csname rrScoredeterministic4\endcsname{12.57}%
\expandafter\def\csname rrScoreflow1\endcsname{8.30}%
\expandafter\def\csname rrScoreflow2\endcsname{8.99}%
\expandafter\def\csname rrScoreflow3\endcsname{9.05}%
\expandafter\def\csname rrScoreflow4\endcsname{9.56}%
\definecolor{rrError0}{rgb}{0.189950,0.071760,0.232170}%
\definecolor{rrError1}{rgb}{0.194830,0.083390,0.261490}%
\definecolor{rrError2}{rgb}{0.199560,0.094980,0.290240}%
\definecolor{rrError3}{rgb}{0.204150,0.106520,0.318440}%
\definecolor{rrError4}{rgb}{0.208600,0.118020,0.346070}%
\definecolor{rrError5}{rgb}{0.212910,0.129470,0.373140}%
\definecolor{rrError6}{rgb}{0.217080,0.140870,0.399640}%
\definecolor{rrError7}{rgb}{0.221110,0.152230,0.425580}%
\definecolor{rrError8}{rgb}{0.225000,0.163540,0.450960}%
\definecolor{rrError9}{rgb}{0.228750,0.174810,0.475780}%
\definecolor{rrError10}{rgb}{0.232360,0.186030,0.500040}%
\definecolor{rrError11}{rgb}{0.235820,0.197200,0.523730}%
\definecolor{rrError12}{rgb}{0.239150,0.208330,0.546860}%
\definecolor{rrError13}{rgb}{0.242340,0.219410,0.569420}%
\definecolor{rrError14}{rgb}{0.245390,0.230440,0.591420}%
\definecolor{rrError15}{rgb}{0.248300,0.241430,0.612860}%
\definecolor{rrError16}{rgb}{0.251070,0.252370,0.633740}%
\definecolor{rrError17}{rgb}{0.253690,0.263270,0.654060}%
\definecolor{rrError18}{rgb}{0.256180,0.274120,0.673810}%
\definecolor{rrError19}{rgb}{0.258530,0.284920,0.693000}%
\definecolor{rrError20}{rgb}{0.260740,0.295680,0.711620}%
\definecolor{rrError21}{rgb}{0.262800,0.306390,0.729680}%
\definecolor{rrError22}{rgb}{0.264730,0.317060,0.747180}%
\definecolor{rrError23}{rgb}{0.266520,0.327680,0.764120}%
\definecolor{rrError24}{rgb}{0.268160,0.338250,0.780500}%
\definecolor{rrError25}{rgb}{0.269670,0.348780,0.796310}%
\definecolor{rrError26}{rgb}{0.271030,0.359260,0.811560}%
\definecolor{rrError27}{rgb}{0.272260,0.369700,0.826240}%
\definecolor{rrError28}{rgb}{0.273340,0.380080,0.840370}%
\definecolor{rrError29}{rgb}{0.274290,0.390430,0.853930}%
\definecolor{rrError30}{rgb}{0.275090,0.400720,0.866920}%
\definecolor{rrError31}{rgb}{0.275760,0.410970,0.879360}%
\definecolor{rrError32}{rgb}{0.276280,0.421180,0.891230}%
\definecolor{rrError33}{rgb}{0.276670,0.431340,0.902540}%
\definecolor{rrError34}{rgb}{0.276910,0.441450,0.913280}%
\definecolor{rrError35}{rgb}{0.277010,0.451520,0.923470}%
\definecolor{rrError36}{rgb}{0.276980,0.461530,0.933090}%
\definecolor{rrError37}{rgb}{0.276800,0.471510,0.942140}%
\definecolor{rrError38}{rgb}{0.276480,0.481440,0.950640}%
\definecolor{rrError39}{rgb}{0.276030,0.491320,0.958570}%
\definecolor{rrError40}{rgb}{0.275430,0.501150,0.965940}%
\definecolor{rrError41}{rgb}{0.274690,0.510940,0.972750}%
\definecolor{rrError42}{rgb}{0.273810,0.520690,0.978990}%
\definecolor{rrError43}{rgb}{0.272730,0.530400,0.984610}%
\definecolor{rrError44}{rgb}{0.271060,0.540150,0.989300}%
\definecolor{rrError45}{rgb}{0.268780,0.549950,0.993030}%
\definecolor{rrError46}{rgb}{0.265920,0.559790,0.995830}%
\definecolor{rrError47}{rgb}{0.262520,0.569670,0.997730}%
\definecolor{rrError48}{rgb}{0.258620,0.579580,0.998760}%
\definecolor{rrError49}{rgb}{0.254250,0.589500,0.998960}%
\definecolor{rrError50}{rgb}{0.249460,0.599430,0.998350}%
\definecolor{rrError51}{rgb}{0.244270,0.609370,0.996970}%
\definecolor{rrError52}{rgb}{0.238740,0.619310,0.994850}%
\definecolor{rrError53}{rgb}{0.232880,0.629230,0.992020}%
\definecolor{rrError54}{rgb}{0.226760,0.639130,0.988510}%
\definecolor{rrError55}{rgb}{0.220390,0.649010,0.984360}%
\definecolor{rrError56}{rgb}{0.213820,0.658860,0.979590}%
\definecolor{rrError57}{rgb}{0.207080,0.668660,0.974230}%
\definecolor{rrError58}{rgb}{0.200210,0.678420,0.968330}%
\definecolor{rrError59}{rgb}{0.193260,0.688120,0.961900}%
\definecolor{rrError60}{rgb}{0.186250,0.697750,0.954980}%
\definecolor{rrError61}{rgb}{0.179230,0.707320,0.947610}%
\definecolor{rrError62}{rgb}{0.172230,0.716800,0.939810}%
\definecolor{rrError63}{rgb}{0.165290,0.726200,0.931610}%
\definecolor{rrError64}{rgb}{0.158440,0.735510,0.923050}%
\definecolor{rrError65}{rgb}{0.151730,0.744720,0.914160}%
\definecolor{rrError66}{rgb}{0.145190,0.753810,0.904960}%
\definecolor{rrError67}{rgb}{0.138860,0.762790,0.895500}%
\definecolor{rrError68}{rgb}{0.132780,0.771650,0.885800}%
\definecolor{rrError69}{rgb}{0.126980,0.780370,0.875900}%
\definecolor{rrError70}{rgb}{0.121510,0.788960,0.865810}%
\definecolor{rrError71}{rgb}{0.116390,0.797400,0.855590}%
\definecolor{rrError72}{rgb}{0.111670,0.805690,0.845250}%
\definecolor{rrError73}{rgb}{0.107380,0.813810,0.834840}%
\definecolor{rrError74}{rgb}{0.103570,0.821770,0.824370}%
\definecolor{rrError75}{rgb}{0.100260,0.829550,0.813890}%
\definecolor{rrError76}{rgb}{0.097500,0.837140,0.803420}%
\definecolor{rrError77}{rgb}{0.095320,0.844550,0.792990}%
\definecolor{rrError78}{rgb}{0.093770,0.851750,0.782640}%
\definecolor{rrError79}{rgb}{0.092870,0.858750,0.772400}%
\definecolor{rrError80}{rgb}{0.092670,0.865540,0.762300}%
\definecolor{rrError81}{rgb}{0.093200,0.872110,0.752370}%
\definecolor{rrError82}{rgb}{0.094510,0.878440,0.742650}%
\definecolor{rrError83}{rgb}{0.096620,0.884540,0.733160}%
\definecolor{rrError84}{rgb}{0.099580,0.890400,0.723930}%
\definecolor{rrError85}{rgb}{0.103420,0.896000,0.715000}%
\definecolor{rrError86}{rgb}{0.108150,0.901420,0.705990}%
\definecolor{rrError87}{rgb}{0.113740,0.906730,0.696510}%
\definecolor{rrError88}{rgb}{0.120140,0.911930,0.686600}%
\definecolor{rrError89}{rgb}{0.127330,0.917010,0.676270}%
\definecolor{rrError90}{rgb}{0.135260,0.921970,0.665560}%
\definecolor{rrError91}{rgb}{0.143910,0.926800,0.654480}%
\definecolor{rrError92}{rgb}{0.153230,0.931510,0.643080}%
\definecolor{rrError93}{rgb}{0.163190,0.936090,0.631370}%
\definecolor{rrError94}{rgb}{0.173770,0.940530,0.619380}%
\definecolor{rrError95}{rgb}{0.184910,0.944840,0.607130}%
\definecolor{rrError96}{rgb}{0.196590,0.949010,0.594660}%
\definecolor{rrError97}{rgb}{0.208770,0.953040,0.581990}%
\definecolor{rrError98}{rgb}{0.221420,0.956920,0.569140}%
\definecolor{rrError99}{rgb}{0.234490,0.960650,0.556140}%
\definecolor{rrError100}{rgb}{0.247970,0.964230,0.543030}%
\definecolor{rrError101}{rgb}{0.261800,0.967650,0.529810}%
\definecolor{rrError102}{rgb}{0.275970,0.970920,0.516530}%
\definecolor{rrError103}{rgb}{0.290420,0.974030,0.503210}%
\definecolor{rrError104}{rgb}{0.305130,0.976970,0.489870}%
\definecolor{rrError105}{rgb}{0.320060,0.979740,0.476540}%
\definecolor{rrError106}{rgb}{0.335170,0.982340,0.463250}%
\definecolor{rrError107}{rgb}{0.350430,0.984770,0.450020}%
\definecolor{rrError108}{rgb}{0.365810,0.987020,0.436880}%
\definecolor{rrError109}{rgb}{0.381270,0.989090,0.423860}%
\definecolor{rrError110}{rgb}{0.396780,0.990980,0.410980}%
\definecolor{rrError111}{rgb}{0.412290,0.992680,0.398260}%
\definecolor{rrError112}{rgb}{0.427780,0.994190,0.385750}%
\definecolor{rrError113}{rgb}{0.443210,0.995510,0.373450}%
\definecolor{rrError114}{rgb}{0.458540,0.996630,0.361400}%
\definecolor{rrError115}{rgb}{0.473750,0.997550,0.349630}%
\definecolor{rrError116}{rgb}{0.488790,0.998280,0.338160}%
\definecolor{rrError117}{rgb}{0.503620,0.998790,0.327010}%
\definecolor{rrError118}{rgb}{0.518220,0.999100,0.316220}%
\definecolor{rrError119}{rgb}{0.532550,0.999190,0.305810}%
\definecolor{rrError120}{rgb}{0.546580,0.999070,0.295810}%
\definecolor{rrError121}{rgb}{0.560260,0.998730,0.286230}%
\definecolor{rrError122}{rgb}{0.573570,0.998170,0.277120}%
\definecolor{rrError123}{rgb}{0.586460,0.997390,0.268490}%
\definecolor{rrError124}{rgb}{0.598910,0.996380,0.260380}%
\definecolor{rrError125}{rgb}{0.610880,0.995140,0.252800}%
\definecolor{rrError126}{rgb}{0.622330,0.993660,0.245790}%
\definecolor{rrError127}{rgb}{0.633230,0.991950,0.239370}%
\definecolor{rrError128}{rgb}{0.643620,0.989990,0.233560}%
\definecolor{rrError129}{rgb}{0.653940,0.987750,0.228350}%
\definecolor{rrError130}{rgb}{0.664280,0.985240,0.223700}%
\definecolor{rrError131}{rgb}{0.674620,0.982460,0.219600}%
\definecolor{rrError132}{rgb}{0.684940,0.979410,0.216020}%
\definecolor{rrError133}{rgb}{0.695250,0.976100,0.212940}%
\definecolor{rrError134}{rgb}{0.705530,0.972550,0.210320}%
\definecolor{rrError135}{rgb}{0.715770,0.968750,0.208150}%
\definecolor{rrError136}{rgb}{0.725960,0.964700,0.206400}%
\definecolor{rrError137}{rgb}{0.736100,0.960430,0.205040}%
\definecolor{rrError138}{rgb}{0.746170,0.955930,0.204060}%
\definecolor{rrError139}{rgb}{0.756170,0.951210,0.203430}%
\definecolor{rrError140}{rgb}{0.766080,0.946270,0.203110}%
\definecolor{rrError141}{rgb}{0.775910,0.941130,0.203100}%
\definecolor{rrError142}{rgb}{0.785630,0.935790,0.203360}%
\definecolor{rrError143}{rgb}{0.795240,0.930250,0.203860}%
\definecolor{rrError144}{rgb}{0.804730,0.924520,0.204590}%
\definecolor{rrError145}{rgb}{0.814100,0.918610,0.205520}%
\definecolor{rrError146}{rgb}{0.823330,0.912530,0.206630}%
\definecolor{rrError147}{rgb}{0.832410,0.906270,0.207880}%
\definecolor{rrError148}{rgb}{0.841330,0.899860,0.209260}%
\definecolor{rrError149}{rgb}{0.850100,0.893280,0.210740}%
\definecolor{rrError150}{rgb}{0.858680,0.886550,0.212300}%
\definecolor{rrError151}{rgb}{0.867090,0.879680,0.213910}%
\definecolor{rrError152}{rgb}{0.875300,0.872670,0.215550}%
\definecolor{rrError153}{rgb}{0.883310,0.865530,0.217190}%
\definecolor{rrError154}{rgb}{0.891120,0.858260,0.218800}%
\definecolor{rrError155}{rgb}{0.898700,0.850870,0.220380}%
\definecolor{rrError156}{rgb}{0.906050,0.843370,0.221880}%
\definecolor{rrError157}{rgb}{0.913170,0.835760,0.223280}%
\definecolor{rrError158}{rgb}{0.920040,0.828060,0.224560}%
\definecolor{rrError159}{rgb}{0.926660,0.820250,0.225700}%
\definecolor{rrError160}{rgb}{0.933010,0.812360,0.226670}%
\definecolor{rrError161}{rgb}{0.939090,0.804390,0.227440}%
\definecolor{rrError162}{rgb}{0.944890,0.796340,0.228000}%
\definecolor{rrError163}{rgb}{0.950390,0.788230,0.228310}%
\definecolor{rrError164}{rgb}{0.955600,0.780050,0.228360}%
\definecolor{rrError165}{rgb}{0.960490,0.771810,0.228110}%
\definecolor{rrError166}{rgb}{0.965070,0.763520,0.227540}%
\definecolor{rrError167}{rgb}{0.969310,0.755190,0.226630}%
\definecolor{rrError168}{rgb}{0.973230,0.746820,0.225360}%
\definecolor{rrError169}{rgb}{0.976790,0.738420,0.223690}%
\definecolor{rrError170}{rgb}{0.980000,0.730000,0.221610}%
\definecolor{rrError171}{rgb}{0.982890,0.721400,0.219180}%
\definecolor{rrError172}{rgb}{0.985490,0.712500,0.216500}%
\definecolor{rrError173}{rgb}{0.987810,0.703300,0.213580}%
\definecolor{rrError174}{rgb}{0.989860,0.693820,0.210430}%
\definecolor{rrError175}{rgb}{0.991630,0.684080,0.207060}%
\definecolor{rrError176}{rgb}{0.993140,0.674080,0.203480}%
\definecolor{rrError177}{rgb}{0.994380,0.663860,0.199710}%
\definecolor{rrError178}{rgb}{0.995350,0.653410,0.195770}%
\definecolor{rrError179}{rgb}{0.996070,0.642770,0.191650}%
\definecolor{rrError180}{rgb}{0.996540,0.631930,0.187380}%
\definecolor{rrError181}{rgb}{0.996750,0.620930,0.182970}%
\definecolor{rrError182}{rgb}{0.996720,0.609770,0.178420}%
\definecolor{rrError183}{rgb}{0.996440,0.598460,0.173760}%
\definecolor{rrError184}{rgb}{0.995930,0.587030,0.168990}%
\definecolor{rrError185}{rgb}{0.995170,0.575490,0.164120}%
\definecolor{rrError186}{rgb}{0.994190,0.563860,0.159180}%
\definecolor{rrError187}{rgb}{0.992970,0.552140,0.154170}%
\definecolor{rrError188}{rgb}{0.991530,0.540360,0.149100}%
\definecolor{rrError189}{rgb}{0.989870,0.528540,0.143980}%
\definecolor{rrError190}{rgb}{0.987990,0.516670,0.138830}%
\definecolor{rrError191}{rgb}{0.985900,0.504790,0.133670}%
\definecolor{rrError192}{rgb}{0.983600,0.492910,0.128490}%
\definecolor{rrError193}{rgb}{0.981080,0.481040,0.123320}%
\definecolor{rrError194}{rgb}{0.978370,0.469200,0.118170}%
\definecolor{rrError195}{rgb}{0.975450,0.457400,0.113050}%
\definecolor{rrError196}{rgb}{0.972340,0.445650,0.107970}%
\definecolor{rrError197}{rgb}{0.969040,0.433990,0.102940}%
\definecolor{rrError198}{rgb}{0.965550,0.422410,0.097980}%
\definecolor{rrError199}{rgb}{0.961870,0.410930,0.093100}%
\definecolor{rrError200}{rgb}{0.958010,0.399580,0.088310}%
\definecolor{rrError201}{rgb}{0.953980,0.388360,0.083620}%
\definecolor{rrError202}{rgb}{0.949770,0.377290,0.079050}%
\definecolor{rrError203}{rgb}{0.945380,0.366380,0.074610}%
\definecolor{rrError204}{rgb}{0.940840,0.355660,0.070310}%
\definecolor{rrError205}{rgb}{0.936120,0.345130,0.066160}%
\definecolor{rrError206}{rgb}{0.931250,0.334820,0.062180}%
\definecolor{rrError207}{rgb}{0.926230,0.324730,0.058370}%
\definecolor{rrError208}{rgb}{0.921050,0.314890,0.054750}%
\definecolor{rrError209}{rgb}{0.915720,0.305300,0.051340}%
\definecolor{rrError210}{rgb}{0.910240,0.295990,0.048140}%
\definecolor{rrError211}{rgb}{0.904630,0.286960,0.045160}%
\definecolor{rrError212}{rgb}{0.898880,0.278240,0.042430}%
\definecolor{rrError213}{rgb}{0.892980,0.269810,0.039930}%
\definecolor{rrError214}{rgb}{0.886910,0.261520,0.037530}%
\definecolor{rrError215}{rgb}{0.880660,0.253340,0.035210}%
\definecolor{rrError216}{rgb}{0.874220,0.245260,0.032970}%
\definecolor{rrError217}{rgb}{0.867600,0.237300,0.030820}%
\definecolor{rrError218}{rgb}{0.860790,0.229450,0.028750}%
\definecolor{rrError219}{rgb}{0.853800,0.221700,0.026770}%
\definecolor{rrError220}{rgb}{0.846620,0.214070,0.024870}%
\definecolor{rrError221}{rgb}{0.839260,0.206540,0.023050}%
\definecolor{rrError222}{rgb}{0.831720,0.199120,0.021310}%
\definecolor{rrError223}{rgb}{0.823990,0.191820,0.019660}%
\definecolor{rrError224}{rgb}{0.816080,0.184620,0.018090}%
\definecolor{rrError225}{rgb}{0.807990,0.177530,0.016600}%
\definecolor{rrError226}{rgb}{0.799710,0.170550,0.015200}%
\definecolor{rrError227}{rgb}{0.791250,0.163680,0.013870}%
\definecolor{rrError228}{rgb}{0.782600,0.156930,0.012640}%
\definecolor{rrError229}{rgb}{0.773770,0.150280,0.011480}%
\definecolor{rrError230}{rgb}{0.764760,0.143740,0.010410}%
\definecolor{rrError231}{rgb}{0.755560,0.137310,0.009420}%
\definecolor{rrError232}{rgb}{0.746170,0.130980,0.008510}%
\definecolor{rrError233}{rgb}{0.736610,0.124770,0.007690}%
\definecolor{rrError234}{rgb}{0.726860,0.118670,0.006950}%
\definecolor{rrError235}{rgb}{0.716920,0.112680,0.006290}%
\definecolor{rrError236}{rgb}{0.706800,0.106800,0.005710}%
\definecolor{rrError237}{rgb}{0.696500,0.101020,0.005220}%
\definecolor{rrError238}{rgb}{0.686020,0.095360,0.004810}%
\definecolor{rrError239}{rgb}{0.675350,0.089800,0.004490}%
\definecolor{rrError240}{rgb}{0.664490,0.084360,0.004240}%
\definecolor{rrError241}{rgb}{0.653450,0.079020,0.004080}%
\definecolor{rrError242}{rgb}{0.642230,0.073800,0.004010}%
\definecolor{rrError243}{rgb}{0.630820,0.068680,0.004010}%
\definecolor{rrError244}{rgb}{0.619230,0.063670,0.004100}%
\definecolor{rrError245}{rgb}{0.607460,0.058780,0.004270}%
\definecolor{rrError246}{rgb}{0.595500,0.053990,0.004530}%
\definecolor{rrError247}{rgb}{0.583360,0.049310,0.004860}%
\definecolor{rrError248}{rgb}{0.571030,0.044740,0.005290}%
\definecolor{rrError249}{rgb}{0.558520,0.040280,0.005790}%
\definecolor{rrError250}{rgb}{0.545830,0.035930,0.006380}%
\definecolor{rrError251}{rgb}{0.532950,0.031690,0.007050}%
\definecolor{rrError252}{rgb}{0.519890,0.027560,0.007800}%
\definecolor{rrError253}{rgb}{0.506640,0.023540,0.008630}%
\definecolor{rrError254}{rgb}{0.493210,0.019630,0.009550}%
\definecolor{rrError255}{rgb}{0.479600,0.015830,0.010550}%
\pgfdeclarehorizontalshading{rrErrorGradient}{100bp}{color(0.000000bp)=(rrError0);color(0.392157bp)=(rrError1);color(0.784314bp)=(rrError2);color(1.176471bp)=(rrError3);color(1.568627bp)=(rrError4);color(1.960784bp)=(rrError5);color(2.352941bp)=(rrError6);color(2.745098bp)=(rrError7);color(3.137255bp)=(rrError8);color(3.529412bp)=(rrError9);color(3.921569bp)=(rrError10);color(4.313725bp)=(rrError11);color(4.705882bp)=(rrError12);color(5.098039bp)=(rrError13);color(5.490196bp)=(rrError14);color(5.882353bp)=(rrError15);color(6.274510bp)=(rrError16);color(6.666667bp)=(rrError17);color(7.058824bp)=(rrError18);color(7.450980bp)=(rrError19);color(7.843137bp)=(rrError20);color(8.235294bp)=(rrError21);color(8.627451bp)=(rrError22);color(9.019608bp)=(rrError23);color(9.411765bp)=(rrError24);color(9.803922bp)=(rrError25);color(10.196078bp)=(rrError26);color(10.588235bp)=(rrError27);color(10.980392bp)=(rrError28);color(11.372549bp)=(rrError29);color(11.764706bp)=(rrError30);color(12.156863bp)=(rrError31);color(12.549020bp)=(rrError32);color(12.941176bp)=(rrError33);color(13.333333bp)=(rrError34);color(13.725490bp)=(rrError35);color(14.117647bp)=(rrError36);color(14.509804bp)=(rrError37);color(14.901961bp)=(rrError38);color(15.294118bp)=(rrError39);color(15.686275bp)=(rrError40);color(16.078431bp)=(rrError41);color(16.470588bp)=(rrError42);color(16.862745bp)=(rrError43);color(17.254902bp)=(rrError44);color(17.647059bp)=(rrError45);color(18.039216bp)=(rrError46);color(18.431373bp)=(rrError47);color(18.823529bp)=(rrError48);color(19.215686bp)=(rrError49);color(19.607843bp)=(rrError50);color(20.000000bp)=(rrError51);color(20.392157bp)=(rrError52);color(20.784314bp)=(rrError53);color(21.176471bp)=(rrError54);color(21.568627bp)=(rrError55);color(21.960784bp)=(rrError56);color(22.352941bp)=(rrError57);color(22.745098bp)=(rrError58);color(23.137255bp)=(rrError59);color(23.529412bp)=(rrError60);color(23.921569bp)=(rrError61);color(24.313725bp)=(rrError62);color(24.705882bp)=(rrError63);color(25.098039bp)=(rrError64);color(25.490196bp)=(rrError65);color(25.882353bp)=(rrError66);color(26.274510bp)=(rrError67);color(26.666667bp)=(rrError68);color(27.058824bp)=(rrError69);color(27.450980bp)=(rrError70);color(27.843137bp)=(rrError71);color(28.235294bp)=(rrError72);color(28.627451bp)=(rrError73);color(29.019608bp)=(rrError74);color(29.411765bp)=(rrError75);color(29.803922bp)=(rrError76);color(30.196078bp)=(rrError77);color(30.588235bp)=(rrError78);color(30.980392bp)=(rrError79);color(31.372549bp)=(rrError80);color(31.764706bp)=(rrError81);color(32.156863bp)=(rrError82);color(32.549020bp)=(rrError83);color(32.941176bp)=(rrError84);color(33.333333bp)=(rrError85);color(33.725490bp)=(rrError86);color(34.117647bp)=(rrError87);color(34.509804bp)=(rrError88);color(34.901961bp)=(rrError89);color(35.294118bp)=(rrError90);color(35.686275bp)=(rrError91);color(36.078431bp)=(rrError92);color(36.470588bp)=(rrError93);color(36.862745bp)=(rrError94);color(37.254902bp)=(rrError95);color(37.647059bp)=(rrError96);color(38.039216bp)=(rrError97);color(38.431373bp)=(rrError98);color(38.823529bp)=(rrError99);color(39.215686bp)=(rrError100);color(39.607843bp)=(rrError101);color(40.000000bp)=(rrError102);color(40.392157bp)=(rrError103);color(40.784314bp)=(rrError104);color(41.176471bp)=(rrError105);color(41.568627bp)=(rrError106);color(41.960784bp)=(rrError107);color(42.352941bp)=(rrError108);color(42.745098bp)=(rrError109);color(43.137255bp)=(rrError110);color(43.529412bp)=(rrError111);color(43.921569bp)=(rrError112);color(44.313725bp)=(rrError113);color(44.705882bp)=(rrError114);color(45.098039bp)=(rrError115);color(45.490196bp)=(rrError116);color(45.882353bp)=(rrError117);color(46.274510bp)=(rrError118);color(46.666667bp)=(rrError119);color(47.058824bp)=(rrError120);color(47.450980bp)=(rrError121);color(47.843137bp)=(rrError122);color(48.235294bp)=(rrError123);color(48.627451bp)=(rrError124);color(49.019608bp)=(rrError125);color(49.411765bp)=(rrError126);color(49.803922bp)=(rrError127);color(50.196078bp)=(rrError128);color(50.588235bp)=(rrError129);color(50.980392bp)=(rrError130);color(51.372549bp)=(rrError131);color(51.764706bp)=(rrError132);color(52.156863bp)=(rrError133);color(52.549020bp)=(rrError134);color(52.941176bp)=(rrError135);color(53.333333bp)=(rrError136);color(53.725490bp)=(rrError137);color(54.117647bp)=(rrError138);color(54.509804bp)=(rrError139);color(54.901961bp)=(rrError140);color(55.294118bp)=(rrError141);color(55.686275bp)=(rrError142);color(56.078431bp)=(rrError143);color(56.470588bp)=(rrError144);color(56.862745bp)=(rrError145);color(57.254902bp)=(rrError146);color(57.647059bp)=(rrError147);color(58.039216bp)=(rrError148);color(58.431373bp)=(rrError149);color(58.823529bp)=(rrError150);color(59.215686bp)=(rrError151);color(59.607843bp)=(rrError152);color(60.000000bp)=(rrError153);color(60.392157bp)=(rrError154);color(60.784314bp)=(rrError155);color(61.176471bp)=(rrError156);color(61.568627bp)=(rrError157);color(61.960784bp)=(rrError158);color(62.352941bp)=(rrError159);color(62.745098bp)=(rrError160);color(63.137255bp)=(rrError161);color(63.529412bp)=(rrError162);color(63.921569bp)=(rrError163);color(64.313725bp)=(rrError164);color(64.705882bp)=(rrError165);color(65.098039bp)=(rrError166);color(65.490196bp)=(rrError167);color(65.882353bp)=(rrError168);color(66.274510bp)=(rrError169);color(66.666667bp)=(rrError170);color(67.058824bp)=(rrError171);color(67.450980bp)=(rrError172);color(67.843137bp)=(rrError173);color(68.235294bp)=(rrError174);color(68.627451bp)=(rrError175);color(69.019608bp)=(rrError176);color(69.411765bp)=(rrError177);color(69.803922bp)=(rrError178);color(70.196078bp)=(rrError179);color(70.588235bp)=(rrError180);color(70.980392bp)=(rrError181);color(71.372549bp)=(rrError182);color(71.764706bp)=(rrError183);color(72.156863bp)=(rrError184);color(72.549020bp)=(rrError185);color(72.941176bp)=(rrError186);color(73.333333bp)=(rrError187);color(73.725490bp)=(rrError188);color(74.117647bp)=(rrError189);color(74.509804bp)=(rrError190);color(74.901961bp)=(rrError191);color(75.294118bp)=(rrError192);color(75.686275bp)=(rrError193);color(76.078431bp)=(rrError194);color(76.470588bp)=(rrError195);color(76.862745bp)=(rrError196);color(77.254902bp)=(rrError197);color(77.647059bp)=(rrError198);color(78.039216bp)=(rrError199);color(78.431373bp)=(rrError200);color(78.823529bp)=(rrError201);color(79.215686bp)=(rrError202);color(79.607843bp)=(rrError203);color(80.000000bp)=(rrError204);color(80.392157bp)=(rrError205);color(80.784314bp)=(rrError206);color(81.176471bp)=(rrError207);color(81.568627bp)=(rrError208);color(81.960784bp)=(rrError209);color(82.352941bp)=(rrError210);color(82.745098bp)=(rrError211);color(83.137255bp)=(rrError212);color(83.529412bp)=(rrError213);color(83.921569bp)=(rrError214);color(84.313725bp)=(rrError215);color(84.705882bp)=(rrError216);color(85.098039bp)=(rrError217);color(85.490196bp)=(rrError218);color(85.882353bp)=(rrError219);color(86.274510bp)=(rrError220);color(86.666667bp)=(rrError221);color(87.058824bp)=(rrError222);color(87.450980bp)=(rrError223);color(87.843137bp)=(rrError224);color(88.235294bp)=(rrError225);color(88.627451bp)=(rrError226);color(89.019608bp)=(rrError227);color(89.411765bp)=(rrError228);color(89.803922bp)=(rrError229);color(90.196078bp)=(rrError230);color(90.588235bp)=(rrError231);color(90.980392bp)=(rrError232);color(91.372549bp)=(rrError233);color(91.764706bp)=(rrError234);color(92.156863bp)=(rrError235);color(92.549020bp)=(rrError236);color(92.941176bp)=(rrError237);color(93.333333bp)=(rrError238);color(93.725490bp)=(rrError239);color(94.117647bp)=(rrError240);color(94.509804bp)=(rrError241);color(94.901961bp)=(rrError242);color(95.294118bp)=(rrError243);color(95.686275bp)=(rrError244);color(96.078431bp)=(rrError245);color(96.470588bp)=(rrError246);color(96.862745bp)=(rrError247);color(97.254902bp)=(rrError248);color(97.647059bp)=(rrError249);color(98.039216bp)=(rrError250);color(98.431373bp)=(rrError251);color(98.823529bp)=(rrError252);color(99.215686bp)=(rrError253);color(99.607843bp)=(rrError254);color(100.000000bp)=(rrError255)}%


==> Images/tikz/reconstruction_violin_style.tex <==
\def\cpviolinmin{3}%
\def\cpviolinmax{1800}%
\def\cpviolinticks{10,30,100,300,1000}%
\definecolor{cpviolinrigid}{HTML}{888888}%
\definecolor{cpviolincompletion}{HTML}{AA4499}%
\definecolor{cpviolindeterministic}{HTML}{D55E00}%
\definecolor{cpviolinindependent}{HTML}{0072B2}%
\definecolor{cpviolinstat}{HTML}{222222}%
\providecommand{\cpviolinmethodlabels}{0/R/rigid,1/C/completion,2/D/deterministic,3/O/independent}%
\providecommand{\cpviolinlabelanchor}{north}%
\providecommand{\cpviolinlabelangle}{0}%
\newcommand{\CPViolin}[7]{%
    \filldraw[draw=#3,fill=#3,fill opacity=.65,draw opacity=.65,line width=.5pt]
        plot file {Images/data/reconstruction_violins/#1_body.dat} -- cycle;
    \draw[only marks,mark=*,mark size=.3pt,draw=#3,fill=#3,opacity=.45,
        mark options={draw=none}]
        plot file {Images/data/reconstruction_violins/#1_tail.dat};
    \draw[cpviolinstat,line width=1.7pt,line cap=round] (#2,#4) -- (#2,#6);
    \filldraw[fill=white,draw=cpviolinstat,line width=.45pt]
        (#2,#5) circle[radius=1.5pt];
    \fill[cpviolinstat] (#2,#7)
        ++(0,1.25pt) -- ++(1.0pt,-1.25pt) -- ++(-1.0pt,-1.25pt)
        -- ++(-1.0pt,1.25pt) -- cycle;
}%
\newcommand{\CPViolinAxis}[8]{%
    \begin{scope}[shift={(#1,#2)},x=#3,y=#4]
    \pgfmathsetmacro{\cplogmin}{ln(#5)/ln(10)}
    \pgfmathsetmacro{\cplogmax}{ln(#6)/ln(10)}
    \pgfmathsetmacro{\cplogspan}{\cplogmax-\cplogmin}
    \edef\cpticklist{#7}
    \foreach \tick in \cpticklist {
        \pgfmathsetmacro{\tickpos}{(ln(\tick)/ln(10)-\cplogmin)/\cplogspan}
        \draw[black!13,line width=.35pt] (0,\tickpos) -- (1,\tickpos);
        \draw[black,line width=.5pt] (0,\tickpos) -- ++(-2pt,0);
        \node[anchor=east,inner sep=0pt,outer sep=0pt]
            at ([xshift=-3.5pt]0,\tickpos) {\tick};
    }
    \pgfmathsetlengthmacro{\cpdatax}{#3/4.16}
    \pgfmathsetlengthmacro{\cpdatay}{#4/\cplogspan}
    \begin{scope}[x=\cpdatax,y=\cpdatay]
        \begin{scope}[shift={(.58,-\cplogmin)}]
            \clip (-.58,\cplogmin) rectangle (3.58,\cplogmax);
            \input{Images/data/reconstruction_violins/#8.tex}
        \end{scope}
    \end{scope}
    \draw[black,line width=.5pt] (0,1) -- (0,0) -- (1,0);
    \foreach \methodindex/\methodletter/\methodcolor in \cpviolinmethodlabels {
        \pgfmathsetmacro{\tickpos}{(\methodindex+.58)/4.16}
        \draw[black,line width=.5pt] (\tickpos,0) -- ++(0,-2pt);
        \node[anchor=\cpviolinlabelanchor,rotate=\cpviolinlabelangle,inner sep=0pt,outer sep=0pt,text=cpviolin\methodcolor,font=\bfseries\fontsize{7}{8.4}\selectfont]
            at ([yshift=-3.5pt]\tickpos,0) {\methodletter};
    }
    \end{scope}%
}%

